S*: Test Time Scaling for Code Generation

Increasing test-time compute for LLMs shows promise across domains but remains underexplored in code generation, despite extensive study in math. In this paper, we propose S*, the first hybrid test-time scaling framework that substantially improves the coverage and selection accuracy of generated code. S* extends the existing parallel scaling paradigm with sequential scaling to push performance boundaries. It further leverages a novel selection mechanism that adaptively generates distinguishing inputs for pairwise comparison, combined with execution-grounded information to robustly identify correct solutions. We evaluate across 12 Large Language Models and Large Reasoning Model and show: (1) S* consistently improves performance across model families and sizes, enabling a 3B model to outperform GPT-4o-mini; (2) S* enables non-reasoning models to surpass reasoning models - GPT-4o-mini with S* outperforms o1-preview by 3.7% on LiveCodeBench; (3) S* further boosts state-of-the-art reasoning models - DeepSeek-R1-Distill-Qwen-32B with S* achieves 85.7% on LiveCodeBench, approaching o1 (high) at 88.5%. Code will be available under https://github.com/NovaSky-AI/SkyThought.

==> intro_shiyi.tex <==
\section{Introduction}
% Increasing the test time compute has been a new trend in increasing LLM performance. As evidenced by the insights from large language monkeys, and the promising results on Math problems in the Deepminds paper.
% v2 --
\DL{Scaling test time compute is an emerging promising direction.}
\textbf{Scaling test-time compute for Large Language Models (LLMs) has increasingly improved their performance}~\citep{openai_learning_to_reason_2024, snell2024scaling, deepseek_r1_lite_2024}. These advancements highlight the potential of leveraging additional computational resources during inference to tackle challenging tasks more effectively. Repeated sampling, for example, can improve coverage by generating diverse attempts, enabling models to solve a higher fraction of problems~\citep{brown2024large}. Beyond repeatedly sampling more samples, there are also other test-time inference methods, such as verification~\citep{} and self-refinement~\citep{madaan2024self}. By effectively allocating test-time compute across these different methods, both scaling efficiency and model performance can improve significantly for complicated tasks such as math reasoning~\citep{snell2024scaling}.


% unique challenges for coding
% todo: make the transition smoother
\DL{Different than existing study in Math, coding problems present unique challenges and opportunities.}
\textbf{While promising, the most effective strategies for scaling test-time compute in competition-level code generation remain largely unexplored}. Similar to math reasoning tasks, test-time inference methods for competition-level code generation can generally be categorized into three phases: generation~\citep{}, self-refinement~\citep{}, and selection~\citep{}, as depicted in \cref{fig:roadmap}. \textbf{However, unlike math reasoning tasks}, where verification heavily relies on high-quality process reward models, such reward models are challenging to obtain for coding tasks~\citep{}. This limitation makes the selection phase significantly more complex for code generation compared to math reasoning. \textbf{Conversely, coding tasks offer a distinct advantage through program execution}, which provides direct feedback on correctness. This unique feature has the potential to substantially enhance the self-refinement phase~\citep{chen2023teaching}, presenting opportunities to optimize test-time performance in ways not available for other reasoning tasks.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{icml2024/figures/roadmap.pdf}
\caption{Roadmap of scaling which dimensions worth scaling.}
\label{fig:roadmap}
\end{figure}


% scaling challenges: 1. scaling behaviour is unclear 2. how to combine these different methods is unclear 
\DL{Previous study on coding has more or less bring up test-time ideas, but no one systematically analyze their scaling behavior.}
\textbf{Moreover, despite a variety of test-time inference methods for code generation}~\citep{chen2022codet}\DL{add cite}, their scaling behavior is poorly understood. For example, sequential sampling -- prompting the LLM to produce multiple answers sequentially -- and parallel strategies like Best-of-N sampling~\citep{} present trade-offs, but their relative efficiency for solving complex coding problems is unclear. In self-refinement, scaling history length risks introducing confounding effects that can degrade performance. For selection, \textbf{key questions remain: is it better to generate many test cases with a weaker model or fewer, higher-quality ones with a stronger model? Does increasing the number of pairwise comparisons consistently improve outcomes}? These challenges highlight the need for a systematic exploration of test-time scaling tailored to the demands of competition-level code generation.




% however, current works 1. only focus more about calling generation diversity, or 2. study the selection policy without studying the scaling effectiveness of these policies.
% Most of the existing works, however, are only focusing on the problem of generation diversity -- although important, it is only one of the key components in complex tasks such as competition-level code generation, where . 


% we are the first work to thoroughly analyze the scaling effectiveness of various mechanisms for all three key stages in the competition-level code generation task.
% .....
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{icml2024/figures/scaling_preview.pdf}
\caption{Scaling curve of~\frameworkname. With the best configuration, we match the performance of o1-preview model.}
\label{fig:scaling_preview}
\end{figure*}

\DL{Our contribution is a systematic study on what dimensions worth scaling in coding problems. Based on the analysis, we set state-of-the-art.}
\textbf{In this paper, we provide the \emph{first} thorough systematic exploration of test-time scaling in competition-level code generation tasks}. We study in-depth 1. the scaling behavior of various test-time inference methods for code generation tasks, and 2. how to combine different test-time inference methods and effectively allocate test-time compute across these methods. Based on our analysis, we develop \frameworkname, a \textbf{compute-optimal} scaling strategy for competition-level code generation tasks%, featuring two new techniques: \textbf{test-aware LLM-as-a-judge} and \textbf{context-aware self-debug}. By leveraging these two techniques,
~\frameworkname~significantly improves model on LiveCodeBench of problems of all different difficulty. Specifically, it improves GPT-4o-mini performance from 78.0 to 95.2 (Easy Problem), 28.2 to 60.2 (Medium problems),  7.3 to 16.7 (Hard problems), exceeding the zero-shot o1-preview model of 92.0, 56.6, and 17.8,  which leverages fine-tuning on private data and potentially a stronger base model. \DL{Potentially add fine-tuned model result to improve: "We discover certain lacking ability that prevent models for more effectively using test-time methods, and fine-tune a model to achieve more effective test-time scaling. Leveraging this model, we further set state-of-the-art.",; can prove this by simply running QwQ as a base model immediately.} \DL{ (1) Add Claude, DeepSeek-2.5-coder, to show the behavior is general. (2) Add two more benchmark, MBPP, (or HumanEval), codecontests; Only need to show the final accuracy.}

==> introduction.tex <==
\section{Introduction}
% Scaling test time is important. There has been quite some work in integrating parallel, sequential, prm, in the math domain. But coding domain has less been explored. This may be due to that . Thus we ask. how can we build the simplest and effective framework to scale coding domain compute effectively?
Scaling test-time compute for Large Language Models (LLMs) has increasingly improved their performance. ~\citet{muennighoff2025s1} introduces 

\joey{
I think the intro is struggling to reverse engineer a problem from the solution. 
Instead, why don't you start by saying that there is a lot of excitement around test-time compute and reasoning capabilities in models.  Then cite \cite{muennighoff2025s1}   as introducing a simple  taxonomy of these techniques and exploring their how to combine these techniques in the context of mathematical reasoning capabilities. (all in the first paragraph)  You then briefly describe their parallel and sequential framing.
Then in the second paragraph you can say in this paper we explore how to combine sequential and parallel scaling in the context of coding tasks. You should then say what is different about coding tasks.  
Then you can jump straight to in this paper we propose frameworkname
}

%\shiyi{Intro outline:
%\begin{enumerate}
%\begin{enumerate}
%    \item Scaling test-time computing is promising.
%    \item What does existing work do? Introduce the commonly used three-stage pipeline.
%    \item However, unlike math, coding presents unique challenges and opportunities within each of these three stages, which remains largely underexplored. Describe the challenges in these three stages.
%    \item To address these challenges, we propose \frameworkname, with optimizations 1, 2, 3, ..., which together boost the performance to xxx.
%    \item Additionally, we conduct a comprehensive ablation study over the large design space to justify our design choices.
%\end{enumerate}
%}
% Increasing the test time compute has been a new trend in increasing LLM performance. As evidenced by the insights from large language monkeys, and the promising results on Math problems in the Deepminds paper.
% v2 --
Scaling test-time compute for Large Language Models (LLMs) has increasingly improved their performance. Mainstream methods often fall into two categories. 
Firstly, \textbf{Sequential} Scaling allows the model to reflect and revise a single Chain-of-thought like solution~\citep{openai_learning_to_reason_2024, deepseek_r1_lite_2024, sky_t1_2025, guo2025deepseek,qwen_qwq_2024}.
\joey{I don't think Sequential Scaling is an established term.  What you are calling sequential scaling is really long chain-of-thought reasoning. None of the citations you listed use this terminology. 
The test-time compute scaling paper refers to sequential sampling but in that case it is re-prompting the model to produce another solution based on the best solution (another way to get Best-of-N) and then picks from the best sequentially generated solutions.  I think actually many people mistakenly attributed reasoning behavior to the test-time compute scaling paper.  This might be because for a while people thought reasoning APIs were running MCTS at inference time.  You could write -- "There has been considerable recent interest in long chain-of-thought reasoning models which leverage significantly increased token generation to improve performance on many challenging benchmarks.  We refer to this form of scaling as Sequential Scaling."  You might want to introduce sequential scaling after parallel scaling? 
Actually, you later cite \cite{muennighoff2025s1} which claims to introduce this terminology on Feb 3rd and does what I proposed here -- renames reasoning behavior as sequential.
}
Secondly, \textbf{Parallel} Scaling repeatedly samples and selects the best solution, often with methods such as Best-of-N~\citep{brown2024large}. 
\begin{figure}[!t]
    \centering
    % First subfigure
    \includegraphics[width=0.45\textwidth]{figures/performance.pdf}      \caption{\textbf{Performance comparison in LiveCodeBench}. ~\frameworkname consistently improves models across different sizes, and both instruction-tuned and newer reasoning models. In particular, ~\frameworkname allows (1) smaller models to outperform 10x larger model: Qwen2.5-3B-Coder-Instruct, integrated with~\frameworkname, outperforms its 32B variant. (2) Older models to outperform newer models: GPT-4o-mini, integrated with~\frameworkname, outperforms O1-Preview. (3) Reasoning models achieve state-of-the-art performance: DeepSeek-R1-Distill-Qwen-32B, integrated with~\frameworkname. outperforms O1-High.}
        \label{fig:performance}
\end{figure}


While both directions have their advantages, they present limitations when we would like to further scale up test-time compute. Firstly, the advantage of sequential scaling eventually flattens out and is limited by the model context window~\citep{muennighoff2025s1}. 
\kurt{awkward; rewrite}
Secondly, even when repeated sampling improves the coverage, the fraction of problem being solved if any of the N samples are correct, the selection method can not always find the correct sample~\citep{brown2024large, stroebl2024inference}. \jx{The second point is a bit hard to get. AND the fraction of problem being solved ...?}
To bridge this gap, hybrid approaches that investigate how to combine parallel and scaling methods have been proposed~\citep{muennighoff2025s1, snell2024scaling}.

\textbf{While hybrid approaches are promising, existing works focus on math domains, due to a wide range of established reward models~\citep{snell2024scaling, muennighoff2025s1}}. 
\joey{Are you saying there is no work on reasoning models for coding tasks?}
The most effective strategies for scaling test-time compute in code generation remain largely unexplored. \jx{Should the 2nd sentence be merged with the 1st sentence and highlighted together?}
Unlike math reasoning tasks, where reward 
signal and selection can be easily derived by exact matching \shangyin{I am not quite convinced by this. What exact-matching signal can we get from an unsolved math problem?}, evaluating coding tasks require large-scale of tests, 
\joey{Do they require large-scale tests?  Couldn't you use a few unit tests to get some signal? Or if you have the solution, just use fuzz testing to verify that the generated solution produced similar results to the ground-truth solution?}
which is scarce in existing datasets~\citep{AceCoder}.
\joey{Several of us are having trouble with the claim that it would be difficult to obtain a reward model for coding tasks.  Do we need to argue this point in the first place? Does there need to be a reason that reasoning models aren't yet applied to coding tasks? Or if there is one then you probably should directly address that in this paper (e.g., propose a reward model).}
This limitation makes the selection phase significantly more complex for code generation compared to math reasoning. On the other hand, coding tasks offer a distinct advantage through program execution, which provides grounded feedback. This characteristics enable self-debug, or potentially reliable selection~\citep{chen2023teaching}.
\jx{Feel that there is a small gap between this para and the next. It is a bit unclear whether we want to address the problem by complementing the dataset or proposing new methods to leverage existing dataset.}

\textbf{In this paper, we propose the first simple hybrid framework~\frameworkname}, to study parallel scaling and sequential scaling strategies of code generation. ~\frameworkname~consists of three phrases that have been proven to be powerful in the context of math problems or partially explored in the coding domain: (1) repeated sampling, which improves overage by generating diverse attempts, enabling models to solve a higher fraction of problems~\citep{brown2024large}, (2) self-debugging,~\citep{chen2023teaching, madaan2024self} on test demonstration, and (3) selection. \jx{We explained the first phases but not the last two. Should we also explain them briefly or removing the explanation of the 1st point to make them aligned?}
We carefully study basic design choice in each axis. Here are the takeaways that enable our final default setting: (1) Parallel: Medium-to-high temperature is sufficient to balance diversity while preserving code quality. We also experiment with several in-context variants but do not observe more significant improvement. (2) Sequential: Self-debug flattens out at usually 2-3 rounds. Interestingly, even strong reasoning models such as R1-7B benefits from real execution. (3) Selection: Majority does not work well; LLM-as-a-judge does not work well by looking at the code; we make a hybrid selection with test-case execution + LLM-as-a-judge with tool-use (i.e., test-case execution) work well. \shangyin{(1) is super clear. (2) and (3) are fuzzy. I think this paragraph could be improved by saying: \frameworkname does (1) (2) and (3), and we observed that they are the best design choices among all.}

% unique challenges for coding
% todo: make the transition smoother
\begin{figure}[th!]
    \centering
    \includegraphics[width=1.0\linewidth]{latex/figures/overview.pdf}
\caption{~\frameworkname~builds on the paradigm of a combination of revision and parallel samples. \jx{Be careful of this because we say we are a three-stage approach.} It first performs a self-refinement on the initial solution to improve algorithm efficiency, and subsequent self-debug round to correct solutions based on public test execution feedback. At the end, it undergoes a selection policy module to select the best solution to output.
\joey{I was confused by this figure as it looks likes Figure 2 from the Snell paper (probably Fig2a).  Does each square reflect a new decode call? It might help to show where teacher-forcing or prompting is done.  Like at the beginning show multiple different prompts to get k different generations. Then show each long context as a tall rectangle and then illustrate the selection process more. }
}
\label{fig:Design}
\end{figure}

We evaluate the effectiveness of~\frameworkname~on ten models across model sizes, open and closed, and both instruction-based or reasoning models.~\frameworkname~has shown consistent improvement, allowing smaller models to outperform 10x larger models, older models to outperform newer models, and reasoning models to set the new state-of-the-art.

In conclusion, our contribution are:
\begin{enumerate}
    \item The first hybrid test-time-scaling framework for code generation.
    \item We study the basic component of each axis with takeaways, provide simple yet strong foundation to be built upon.
    \item We extensively evaluate the effectivenes of our framework, with ablations on detailed design choice. Our framework improves xxx...
    \item We will open-source all softward artifacts, as well as all model generation, intermediates results to facilitate the community research.
\end{enumerate}

\dacheng{(1) simulate cases without unite tests}
~\dacheng{Seems like missing : coding community has not really look at how to scale these little components, like tuning temperature versus ICL, diversity favor, scaling self-debug round. They mostly do look at how to do selection (but not our test+LLM hybrid selection).}



==> method.tex <==
\begin{figure}[!t]
    \centering
    % First subfigure
    \includegraphics[width=0.45\textwidth]{figures/breakdown.pdf}      \caption{\textbf{Example overview of performance.}}
        \label{fig:breakdown}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{icml2024/figures/scaling_preview.pdf}
\caption{Scaling curve of~\frameworkname. With the best configuration, we match the performance of o1-preview model. \shangyin{what model is this?}}
\label{fig:scaling_preview}
\end{figure*}

% unique challenges for coding
% todo: make the transition smoother
\begin{figure}[th!]
    \centering
    \includegraphics[width=1.0\linewidth]{latex/figures/overview.pdf}
\caption{~\frameworkname~builds on the paradigm of a combination of revision and parallel samples. \jx{Be careful of this because we say we are a three-stage approach.} It first performs a self-refinement on the initial solution to improve algorithm efficiency, and subsequent self-debug round to correct solutions based on public test execution feedback. At the end, it undergoes a selection policy module to select the best solution to output.
\joey{I was confused by this figure as it looks likes Figure 2 from the Snell paper (probably Fig2a).  Does each square reflect a new decode call? It might help to show where teacher-forcing or prompting is done.  Like at the beginning show multiple different prompts to get k different generations. Then show each long context as a tall rectangle and then illustrate the selection process more. }
}
\label{fig:Design}
\end{figure}

\section{Method}
\label{sec:method}
In this section, we formally introduce our framework~\frameworkname. ~\frameworkname~takes in a coding problem $\mathbf{P}$, and a model $\mathbf{M}$. The model $\mathbf{M}$ attempts to a program solution $\mathbf{S(\cdot)}$ to maps an input to an output following the problem specification.

In our setup, a coding problem $\mathbf{P}$ contains a problem description in natural language. It contains two sets of test cases in the format of input and expected output: public test $T_{public} = \{(I_i, O_i)\}_{i=1}^{k_{public}}$, and private test $T_{private} = \{(I_i, O_i)\}_{i=1}^{k_{private}}$. Public tests are available to $\mathbf{M}$ to clarify the intent of the natural language description. Private tests are not available to $\mathbf{M}$. The solution is correct if $\mathbf{S}$ passes all the private tests, i.e. if $S(I_i) = O_i, \forall i = 1, ..., k_{private}$. This formulation has been proposed in benchmarks such as~\citet{chen2021evaluating, li2022competition, li2023taco, jain2024livecodebench, hendrycksapps2021, gulwani4foundations}. This is in contrast to math problems, where no additional information is given beyond the problem specification, and evaluation is done by exact matching on the final solution.


% In this section, we formally introduce the problem setup and the ~\frameworkname~framework. %an experiment setup to configure the default setting that we will use in our final experiment.
% \joey{I wouldn't add the experiment setup in the methods section.}


%\noindent\textbf{Problem Setup} We consider coding problems that are clearly specified and unambiguous, as pointed out to be important in~\citet{chowdhury2024introducing}. In particular, we assume coding problems that include a small amount of input and output demonstrations, a common setup as~\citep{chen2021evaluating, li2022competition, li2023taco, jain2024livecodebench, hendrycksapps2021, gulwani4foundations}. We provide one such example in~\autoref{sec:appendix_example_code}. \joey{This paragraph doesn't actually say much. Instead, you might say something that is more detailed and provides greater contrast to the math setting.  In the programming setting we are given a detailed description of a function to implement along with a set of $k$? test input-output pairs and asked to produce a program that produces the same output for each test input.  The model then produces an implementation that is evaluated on a hidden set of unit-tests.  This is in contrast to the math setting where no additional information is given beyond the problem statement and evaluation is done by exact matching on the final solution.}

\subsection{\frameworkname}
\frameworkname~is a two-stage framework: Generation stage and Selection stage.
The generation stage leverages parallel sampling to improve coverage, the fraction of problems that could be solved, jointly with self debugging from public tests to control the quality of such diverse samples~\autoref{sec:scale_parallel_samples}. The selection stage features a test-assisted LLM-as-a-judge approach, which leverages code execution to provide further information to enable accurate LLM evaluation (~\autoref{sec:scale_selection}).

% \frameworkname~is a simple and effective three-stage approach. 
%\joey{I don't think you need the words simple and effective.  They are okay in the intro but here just say it is a three stage approach that combines sequential and parallel scaling with a verification process.  Then provide a high-level description of each of the three phases and how they work together.  It should be clear at the end that this is simple and in the eval you will prove it is effective.}
% It incorporates the advantage of parallel scaling by allowing the model to generate multiple solutions to improve coverage~\citep{brown2024large}, sequential scaling by allowing the model to revise a previous code solution by providing execution feedback on available public demonstration, and that of a verifier by choosing the best one. A high-level illustration can be found at~\autoref{fig:Design}. % In this section, we will introduce each stage, and our findings based on a development set to enable the default setting of~\frameworkname.

\subsubsection{Stage 1: Generation}
% \section{Scaling Parallel Sampling}
\label{sec:scale_parallel_samples}
In the generation stage,~\frameworkname~integrates repeated sampling with the SELF-DEBUGGING approach. The model $\mathbf{M}$ first generates $\mathbf{N}$ coding solutions in parallel. Then perform SELF-DEBUGGING of these $\mathbf{N}$ samples independently. For each sample, if it passes $T_{publlic}$, then it exits for the selection phrase.








Recent work suggests that drawing multiple candidate solutions from language models can substantially improve the final result by increasing coverage of the solution space~\citep{brown2024large, li2022competition}. In this section, we evaluate how sampling many times in parallel scales performance across tasks of varying difficulty (Easy, Medium, Hard), under different temperatures, and with or without in-context examples. 
We adopt an \textit{oracle verifier} (i.e., the checker is assumed perfect) to isolate the effect of sampling itself, following the recommendations of \citet{stroebl2024inference}.
\joey{We only adopt the oracle in the evaluation? Does the method also assume an oracle?}

\paragraph{Repeated Sampling Improves Accuracy, even for reasoning models.}
Table~\ref{tab:sec4_vanilla-temp07} shows that, for \textbf{easy} problems, all models eventually reach nearly 100\% accuracy given sufficient samples (often by \(n=64\)). For instance, \textit{gpt-4o-mini} jumps from 80.7\% at \(n=1\) to 100\% by \(n=8\), and QwQ-32B-Preview achieves 100\% by \(n=2\). Meanwhile, on \textbf{medium} problems, stronger models exhibit larger gains, e.g., \textit{gpt-4o-mini} improves from 32.4\% at \(n=1\) to 70.3\% at \(n=128\), whereas a weaker model like \textit{Qwen2.5-Coder-7B-Instruct} moves from 8.1\% to 51.4\%. \textbf{Hard} problems benefit as well, albeit starting from low baselines; for example, \textit{Qwen2.5-Coder-32B-Instruct} rises from 2.04\% to 14.3\% by sampling 128 times. Interestingly, our preliminary experiments on a more recent reasoning-oriented model (\textit{QwQ-32B-Preview}) reveal a similar pattern: it scales from 4.08\% to 32.65\% on hard problems once sampled 64 times.

\paragraph{Medium temperature (0.7) improves performance, but higher temperature hurts (0.95).} To examine the influence of temperature on parallel sampling, we vary this parameter and present the results in Table~\ref{tab:temp-various}. Moderate temperatures (e.g., 0.2 to 0.7) typically yield performance improvements by promoting greater diversity among the generated samples. However, once temperature surpasses approximately 0.7, performance tends to deteriorate—likely due to the introduction of excessive noise. For example, while \textit{gpt-4o-mini} attains a notable increase in \textbf{hard} task accuracy (from 2.04\% at 0.2 to 8.16\% at 0.95), the gains observed in medium-difficulty tasks do not follow an equally consistent upward trend. Indeed, some models experience performance regressions at higher temperatures, underscoring the trade-off between sampling diversity and solution consistency.

\paragraph{Using relevant in-context examples enhances generation diversity and performance.} 

Furthermore, we investigate whether augmenting prompts with various in-context examples improves parallel sampling. Our example set consists of 362 coding problems with correct solutions and reasoning generated by GPT-4o mini. We design two retrieval approaches for selecting examples. The first, \emph{ICL (BM25)}, uses a BM25 retriever to fetch the top-$k$ similar prompts and prepend each distinct one to different samples when $n = k$. While straightforward, this method may overlook semantics and fail to capture solution-level similarities. To address this, our second approach, \emph{ICL (Pattern)}, categorizes problems based on recurring solution techniques (e.g., dynamic programming) and retrieves examples of the same type. This pattern-based method aims to provide more relevant and structurally similar examples.

\begin{figure*}[ht]
    \centering
    % Placeholder figure
    \includegraphics[width=.8\linewidth]{latex/figures/icl_results.pdf}
    \caption{Performance on medium coding problems with varying numbers of parallel samples (\(n\)) across different methods: Zero-Shot, ICL (BM25), and ICL (Pattern). The results are shown for three models: GPT-4o-mini, Qwen2.5-Coder-7B-Instruct, and Qwen2.5-Coder-32B-Instruct.}
    \label{fig:icl_performance}
\end{figure*}

% Our preliminary findings suggest negligible or inconsistent gains, potentially due to limited marginal improvements in solution diversity once the model already samples multiple times. Further analysis of \emph{token usage} and \emph{response diversity} is underway to clarify whether reasoning-style prompts might yield greater benefit from parallel sampling compared to simpler, non-reasoning tasks.

\ref{tab:icl} and \ref{tab:diversity} demonstrate that selecting in-context examples increases response diversity, and 

\xiuyu{Will write results analysis -- takeaways beyond inconsistent performance improvements (difficulty to construct and retrieve useful examples, model dependent, relation to diversity and number of samples etc.). Future directions could be using a larger, more diverse, more relevant ICL examples database, or design more sophisticated retrieval pipeline.}

Overall, these results reinforce the value of parallel sampling in improving coverage and final accuracy, highlighting (i) the substantial gains on harder tasks achieved by stronger models, (ii) the beneficial but nuanced effect of temperature, and (iii) the complexity and potential limits of simple in-context approaches in further boosting parallel sampling.

\begin{table}[ht]
\centering
\small
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l l r r r r r r r r}
\toprule
\textbf{Model} & \textbf{Difficulty} 
   & \textbf{n=1} & \textbf{n=2} & \textbf{n=4} & \textbf{n=8} 
   & \textbf{n=16} & \textbf{n=32} & \textbf{n=64} & \textbf{n=128} \\
\midrule
\multirow{3}{*}{gpt-4o-mini} 
 & Easy   & 80.7 & 88.5 & 92.3 & 100  & 100  & 100  & 100  & 100  \\
 & Medium & 32.4 & 37.8 & 46.0 & 48.9 & 56.8 & 64.9 & 67.5 & 70.3 \\
 & Hard   & 0.0  & 0.0  & 2.04 & 2.04 & 2.04 & 2.04 & 4.08 & 6.12 \\
\midrule
\multirow{3}{*}{Qwen2.5-Coder-7B-Instruct} 
 & Easy   & 46.2 & 65.4 & 76.9 & 84.6 & 88.5 & 96.2 & 100  & 100  \\
 & Medium & 8.1  & 18.9 & 21.6 & 32.4 & 40.5 & 46.0 & 51.4 & 51.4 \\
 & Hard   & 2.04 & 2.04 & 2.04 & 2.04 & 2.04 & 2.04 & 2.04 & 4.08 \\
\midrule
\multirow{3}{*}{Qwen2.5-Coder-32B-Instruct} 
 & Easy   & 75.9 & 84.6 & 96.2 & 100  & 100  & 100  & 100  & 100  \\
 & Medium & 35.1 & 37.8 & 43.2 & 48.9 & 51.4 & 54.1 & 59.5 & 62.1 \\
 & Hard   & 2.04 & 6.12 & 6.12 & 8.16 & 10.2 & 10.2 & 10.2 & 14.3 \\
\midrule
\multirow{3}{*}{QwQ-32B-Preview} 
 & Easy   & 84.6 & 100  & 100  & 100  & 100  & 100  & 100  & 100  \\
 & Medium & 43.2 & 54.5 & 75.7 & 86.5 & 86.5 & 91.9 & 91.9 & R    \\
 & Hard   & 4.08 & 20.4 & 16.3 & 22.45 & 24.5 & 32.65 & R   & R    \\
\bottomrule
\end{tabular}
}
\caption{Vanilla --- temp=0.7. The effect of repeated sampling on Easy, Medium, and Hard tasks across different models.
\joey{Can we make this three line plots (Easy, Medium, Hard) with $n$ as the x axis.  Show markers (with numbers) and use log-scale on the x-axis. Each model should be a different line.}
}
\label{tab:sec4_vanilla-temp07}
\end{table}

\begin{table}[ht]
\centering
\small
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l l r r r r}
\toprule
\textbf{Model} & \textbf{Difficulty} & 
\textbf{temp=0.2} & \textbf{temp=0.5} & \textbf{temp=0.7} & \textbf{temp=0.95} \\
\midrule

%============= GPT-4o-mini
\multirow{3}{*}{\begin{tabular}{c}
gpt-4o-\\
mini
\end{tabular}}
 & Easy   & 100   & 100   & 100   & 100   \\
 & Medium & 59.5  & 64.8  & 70.3  & 70.3  \\
 & Hard   & 2.04  & 4.10  & 6.12  & 8.16  \\
\midrule

%============= Qwen2.5-Coder-7B-Instruct
\multirow{3}{*}{\begin{tabular}{c}
Qwen2.5-Coder-\\
7B-Instruct
\end{tabular}}
 & Easy   & 80.8  & 96.2  & 100   & 100   \\
 & Medium & 37.9  & 51.4  & 51.4  & 48.9  \\
 & Hard   & 2.04  & 2.04  & 4.08  & 2.04  \\
\midrule

%============= Qwen2.5-Coder-32B-Instruct
\multirow{3}{*}{\begin{tabular}{c}
Qwen2.5-Coder-\\
32B-Instruct
\end{tabular}}
 & Easy   & 100   & 100   & 100   & 100   \\
 & Medium & 54.1  & 62.2  & 62.1  & 65.0  \\
 & Hard   & 10.2  & 12.24 & 14.3  & 12.2  \\
\midrule
\end{tabular}
} 
\caption{Effect of temperature: benefits are observed up to around 0.7, but performance may drop with higher temperature (0.95).
\joey{Can we make this a line plot following the same setup in as proposed for Table 1.}
}
\label{tab:temp-various}
\end{table}

\textbf{Code Diversity} Use execution to cluster responses, measure corresponding final results. % \DL{@xiuyu will help}

%\textbf{Token Efficiency} \textbf{@Shiyi:} Whether QwQ is worth it.
%\DL{Soon}

\subsubsection{Stage 2: Sequential Scaling}
\label{sec:scale_revision}

\paragraph{Setting Description.}
To explore the potential of revision, we leverage the self-debug paradigm~\citep{chen2023teaching}, which executes the generated code on the public tests, and ask the LLMs to further debug based on the error messages. We study three self-debug paradigms in this section - the vanilla one which simply appends the context with new error messages. Last-Round: which only uses the code and error fround the last round of self-debug, to avoid problems such as lost-in-the-middle. Generated tests - public tests can only cover a small portion of tests, we further generate AI-tests to debug according to AlphaCodium. We use 8 parallel samples and assume an oracle verifier in this section.

\DL{Messages:
1. Similar effect of self-debug and scaling samples. e.g. spending 4x more compute on self-debugging gpt-4o-mini improves 13\% while 16\% in parallel samples.
2. Self-debug techniques quickly saturated in 3-4 rounds. Easier problems require fewer rounds to reach upper bound.
3. Further debugging on generated tests or managing context do not improve result.
}
\paragraph{Usefulness of Self-Debugging.}
We first examine how well self-debugging improves performance and how it compares to repeated sampling across different scenarios. As shown in Table~\ref{tab:revision_comparison}, allowing the model to iteratively refine its output (\emph{Vanilla} approach) can yield appreciable gains on \textbf{easy} and, to a lesser extent, \textbf{medium} tasks. For example, \textit{gpt-4o-mini} improves from 96.2\% at \(r=0\) to 100\% by \(r=1\) on easy problems, while \textit{Qwen2.5-Coder-32B-Instruct} moves from 45.9\% to 59.5\% on medium tasks. However, all models struggle with \textbf{hard} tasks: even multiple rounds of refinement tend to yield only marginal gains (e.g., 2.04\% to 4.08\% or 6.12\%, see also \S\ref{sec:scale_parallel_samples} for parallel sampling results). In practice, repeated sampling often provides broader coverage of potential solutions, whereas self-debugging helps refine an existing candidate. The two methods can complement each other, though our findings indicate that repeated sampling alone is frequently more impactful on harder items.

\subsubsection{Selection}
\label{sec:scale_selection}
After Stage 2, there are N samples that needed to be selected. In this section, we consider several ways to do this selection, and propose our simple solution to better select candidates. We consider the following algorithms.

\paragraph{Generated tests based} The most straightforward way to do selection is to do majority voting. Unlike math domains, where results are matched by exact match, in coding, we need to generate test inputs -> Generated test inputs + majority voting on the output. The other way is to do generated inputs and generated test outputs, also a popular choice~\citep{ehrlich2025codemonkeys}.

\paragraph{LLM-as-a-judge based} This is often used in natural language as the way to select the better samples.


Some ablation here - we find that generated tests + majority voting is not reliable because majority is wrong for hard problems. Using test outputs are also wrong because usually that assumes a strong model.

On the other hand, LLM-as-a-judge can not found the correct one, because llm can hardly reason on code.

Based on this, we develope a hybrid approach, shown in some figure, that first uses test inputs to cluster into several groups. then we use llm-as-a-judge. However, we do not simply use llm-as-a-judge, as we know it does not work. We let the llm to propose a test input that can potentially distinguish samples, execute it back, and then based on the results, do the selection, We found this consistently improve the result.\DL{Add figure, and a table here.}


==> new_intro.tex <==
\section{Introduction}
% Scaling test time is important. There has been quite some work in integrating parallel, sequential, prm, in the math domain. But coding domain has less been explored. This may be due to that . Thus we ask. how can we build the simplest and effective framework to scale coding domain compute effectively?
Scaling test time compute is highly effective in improving the performance of Large Language Models (LLMs)~\citep{openai_learning_to_reason_2024, guo2025deepseek,qwen_qwq_2024,muennighoff2025s1,sky_t1_2025,brown2024large,snell2024scaling}. 
In math reasoning tasks, in particular, extensive research has explored various test-time scaling strategies, including repeated sampling to improve solution coverage~\citep{ehrlich2025codemonkeys}, iterative refinement through rethinking and revising previous solutions, and the use of reward models to provide more effective guidance in the search process~\citep{snell2024scaling, li2024rethinkmcts}. 

While significant progress has been made in math reasoning tasks, test-time scaling for code generation---an essential domain with wide-ranging applications---remains largely underexplored.
Unlike math reasoning tasks, where correctness can often be verified by exact string matching~\cite{}, \jx{Need a citation}
checking correctness in coding tasks requires executing a large scale of test cases to increase accuracy~\citep{liu2023your}, adding complexity to the test time framework and the potential reward model feedback~\citep{AceCoder}. 
On the other hand, coding tasks offer a unique advantage: they can leverage existing language interpreters to generate precise outputs for the given program and inputs. This capability provides a reliable grounding for revising or selecting solutions~\citep{chen2023teaching}.

\iffalse
Scaling test time compute for Large Language Models (LLMs) has increasingly improved model performance~\citep{openai_learning_to_reason_2024, guo2025deepseek,qwen_qwq_2024,muennighoff2025s1,sky_t1_2025,brown2024large,snell2024scaling}. In math reasoning tasks, a rich line of literature has studied how to use repeated sampling to improve coverage~\citep{ehrlich2025codemonkeys}, rethinking and revising previous solutions, and reward models to provide accurate guidance in a searching process~\citep{snell2024scaling, li2024rethinkmcts}. While there has been great success in the math reasoning domain, the code generation domain has been largely under-explored. Unlike the math domain where correctness can be easily checked by exact string matching, correctness in coding tasks requires executing a large scale of test cases to avoid false positives~\citep{liu2023your}, complicating test time framework, and potential reward model feedback~\citep{AceCoder}. On the other hand, coding tasks can leverage interpreter, which provides accurate output given a coding program and an input. This can potentially provide grounding for revising or selecting solutions~\citep{chen2023teaching}.
% test cases with execution, which can potentially provide some grounding as reward models.
\fi

% Thus, in this paper, we ask: \textit{how can we build the simplest framework to scale test time compute in for the coding domain effectively?}
\begin{figure}[!t]
    \centering
    % First subfigure
    \includegraphics[width=0.49\textwidth]{figures/diff_model_performance.pdf}      \caption{\textbf{Performance improvement with~\frameworkname~in LiveCodeBench}. "Qwen-Coder" denotes "Qwen2.5-Coder-Instruct", "R1-Distill" denotes "DeepSeek-R1-Distill-Qwen".~\frameworkname consistently improves models across different sizes, allowing non-reasoning models to surpass reasoning models, and open models to be competitive to o1 (high reasoning effort).}%.\dacheng{run o1-high}}
    \label{fig:all_models_performance}
\end{figure}
%\begin{figure}[!t]
%    \centering
    % First subfigure
    %\includegraphics[width=0.45\textwidth]{figures/performance.pdf}      \caption{\textbf{Performance comparison in LiveCodeBench}. ~\frameworkname consistently improves models across different sizes, and both instruction-tuned and newer reasoning models. In particular, ~\frameworkname allows (1) smaller models to outperform 10x larger model: Qwen2.5-3B-Coder-Instruct, integrated with~\frameworkname, outperforms its 32B variant. (2) Older models to outperform newer models: GPT-4o-mini, integrated with~\frameworkname, outperforms O1-Preview. (3) Reasoning models achieve state-of-the-art performance: DeepSeek-R1-Distill-Qwen-32B, integrated with~\frameworkname. outperforms O1-High.}
       % \label{fig:performance}
%\end{figure}

% In this paper, we propose \frameworkname, the first hybrid test-time scaling framework that substantially improves the coverage and selection accuracy of the generated code. \frameworkname extends the existing parallel scaling paradigm with sequential scaling to further push the upper bound and leverages a novel selection mechanism that combines LLM-based evaluation with execution-grounded verification to robustly identify correct solutions.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{latex/figures/overview_new.pdf}
\caption{\frameworkname builds on the paradigm of a combination of revision and parallel samples. 
It first performs a self-refinement on the initial solution to improve algorithm efficiency, and subsequent self-debug round to correct solutions based on public test execution feedback. At the end, it undergoes a selection policy module to select the best solution to output.
% \joey{I was confused by this figure as it looks likes Figure 2 from the Snell paper (probably Fig2a).  Does each square reflect a new decode call? It might help to show where teacher-forcing or prompting is done.  Like at the beginning show multiple different prompts to get k different generations. Then show each long context as a tall rectangle and then illustrate the selection process more. }
}
\label{fig:Design}
\end{figure*}

In this paper, we introduce \frameworkname, the first hybrid test-time scaling framework for coding tasks, which significantly enhances the coverage and quality of generated code.
\frameworkname has two stages, as illustrated in Figure~\ref{fig:Design}.
In the generation stage, \frameworkname extends parallel scaling (i.e., repeated sampling)~\citep{brown2024large, li2022competition} by incorporating sequential scaling with \textit{iterative debugging}, enhancing both code coverage and quality.
Specifically, for each parallel sample, \frameworkname executes the generated code on public test cases using the corresponding language interpreter to obtain accurate outputs and/or error messages. These outputs and error messages are then fed back to the model, enabling it to iteratively revise the code and generate improved samples.
Interestingly, we find that even for reasoning models that already perform hypothetical debugging during the thinking process, iterative debugging with actual code execution, along with output and error message feedback, can further significantly enhance their performance.~\dacheng{add a small section in experiments to cite}


\iffalse
In this paper, we develop a two-stage approach,  which we call \frameworkname, that leverages test cases and execution to provide grounding information to scale the test time compute for LLMs effectively.
%\textbf{In this paper, we propose the first simple hybrid framework~\frameworkname}, to study parallel scaling and sequential scaling strategies of code generation.
\shiyi{}
In the generation stage, \frameworkname leverages repeated sampling~\citep{brown2024large, li2022competition} to generate solutions in parallel, enabling models to generate multiple coding candidates.
% \joey{finish this sentence}
In contrast to prior work that based on repeated sampling~\citep{brown2024large, li2022competition}, we find that performing further revision on public test cases significantly improves the quality of these candidates. 
Interestingly, we find that even reasoning models, which already perform hypothetical debugging during the thinking process, also benefit significantly from additional debugging iterations~\dacheng{add a small section in experiments to cite}. 
\fi

For sample selection, we find that existing approaches, which blindly generate test inputs for all samples, fail to accurately distinguish between pairwise samples. To address this limitation, we propose \textit{adaptive input synthesis}. Specifically, for each pair of samples, we prompt an LLM to generate test inputs that can effectively differentiate them. Then, by executing the samples with these inputs, we select the best-performing sample based on the actual execution results.


\iffalse
We also explore several approaches to the selection stage. 
We find that the commonly used majority voting  and LLM-as-a-judge based approaches to select the correct solution perform poorly in the code generation setting.
Thus, we develop a novel test-assisted LLM-as-a-judge approach, where an LLM is prompted to generate distinguishing inputs on which the code is run.  The LLM-as-a-judge is then given the input-output pairs along with the code to make a more informed decision about correctness.
\fi


% three phrases that have been proven to be powerful in the context of math problems or partially explored in the coding domain: (1) repeated sampling, which improves overage by generating diverse attempts, enabling models to solve a higher fraction of problems~\citep{brown2024large}, (2) self-debugging,~\citep{chen2023teaching, madaan2024self} on test demonstration, and (3) selection. %\jx{We explained the first phases but not the last two. Should we also explain them briefly or removing the explanation of the 1st point to make them aligned?}
% We carefully study basic design choice in each axis. Here are the takeaways that enable our final default setting: (1) Parallel: Medium-to-high temperature is sufficient to balance diversity while preserving code quality. We also experiment with several in-context variants but do not observe more significant improvement. (2) Sequential: Self-debug flattens out at usually 2-3 rounds. Interestingly, even strong reasoning models such as R1-7B benefits from real execution. (3) Selection: Majority does not work well; LLM-as-a-judge does not work well by looking at the code; we make a hybrid selection with test-case execution + LLM-as-a-judge with tool-use (i.e., test-case execution) work well. % \shangyin{(1) is super clear. (2) and (3) are fuzzy. I think this paragraph could be improved by saying: \frameworkname does (1) (2) and (3), and we observed that they are the best design choices among all.}



% We found xxx works

% We conduct xxx

% Our contribution is xxx

We evaluate \frameworkname on 12 models across model sizes, open and closed, and both instruction-based or reasoning models. \frameworkname has shown consistent improvement over zero-shot generation or existing popular test-time scaling methods. In particular, \frameworkname~allows (1) small models to outperform large models in the same family: Qwen2.5-7B-Instruct + \frameworkname outperforms Qwen2.5-32B-Instruct on LiveCodeBench by 10.7\%; (2) instruction-based model to outperform reasoning models: GPT-4o-mini + \frameworkname outperforms o1-preview by 3.7\%; 
and (3) open reasoning models to perform competitively to the state-of-the-art: DeepSeek-R1-Distill-Qwen-32B + \frameworkname~ achieves 85.7\% on LiveCodeBench, where the state-of-the-art (o1-high) is 88.7\%.
Figure~\ref{fig:breakdown} shows an example overview of the benefits of our proposed techniques.
We further include comprehensive ablation studies on 
% different selection methods, 
% the effect of temperature tuning during the generation phase, 
% the impact of using in-context retrieval methods, 
variants of iterative debugging and selection methods in the experiment section~\ref{sec:exp}.

In conclusion, our contributions are:
\begin{enumerate}
\item The first hybrid test-time scaling framework that extends parallel scaling by incorporating sequential scaling with iterative debugging for high code coverage and uses LLMs to adaptively synthesize test inputs for accurate best sample selection. 
%    \item The first hybrid test-time-scaling framework for code generation.
\item We perform extensive evaluation on LiveCodeBench and CodeContests, and show that \frameworkname consistently improve performance across model families and sizes.
%with ablations on detailed design choice. Our framework improves xxx...
\item We will open-source all software artifacts, as well as model generations and intermediates results to facilitate the research community.
\end{enumerate}

\iffalse
In conclusion, our contributions are:
\begin{enumerate}
\item A framework that incorporates repeated sampling with revision from test execution result, LLM selection with code execution result to effectively leverage test-time compute to improve code generation.
%    \item The first hybrid test-time-scaling framework for code generation.
\item We perform extensive evaluation on LiveCodeBench and CodeContests, and show that \frameworkname consistently improve performance across model sizes.
%with ablations on detailed design choice. Our framework improves xxx...
\item We will open-source all software artifacts, as well as model generations and intermediates results to facilitate the research community.
\end{enumerate}
\fi

\begin{figure}[!t]
    \centering
    % First subfigure
    \includegraphics[width=1.0\linewidth]{figures/breakdown_new.pdf}      \caption{\textbf{Example overview of performance.} 
    % \jx{We can potentially replace the non-reasoning model to beat o1-preview.}
}
        \label{fig:breakdown}
\end{figure}


==> new_method.tex <==
% unique challenges for coding
% todo: make the transition smoother
\section{Method}
\label{sec:method}
In this section, we introduce our framework. ~\frameworkname~takes in a coding problem $\mathbf{P}$, and a code generation model $\mathbf{M}$. 
The model $\mathbf{M}$ attempts to generate a program solution $\mathbf{S(\cdot)}$ to maps an input to an output following the problem specification.%\joey{This sentence seems broken.}

In this work, we follow the standard coding framework adopted by most benchmarks~\citep{chen2021evaluating, li2022competition, li2023taco, jain2024livecodebench, hendrycksapps2021, gulwani4foundations}.
Each coding problem $\mathbf{P}$ consists of a problem description in natural language along with set of public and private test cases. 
The test cases are in the form of input-output pairs. 
%There are typically \joey{add number} public test cases and \joey{add number} private test cases.
% and expected output pair: public test $T_\text{public} = \{(I_i, O_i)\}_{i=1}^{k_\text{public}}$, and private test $T_\text{private} = \{(I_i, O_i)\}_{i=1}^{k_\text{private}}$. 
Private tests are not available to $\mathbf{M}$ and are instead used to score the mode on the benchmark. 
The solution is correct if $\mathbf{S}$ passes all the private tests. In contrast, the public tests are available to $\mathbf{M}$ to clarify the intent of the natural language description and are typically included in the prompt. The number of public tests are usually much less than that of private tests. For instance, in CodeContests~\citep{li2022competition}, there are on average 2.0 public tests and 202.1 private tests per problem.
% i.e., if $S(I_i) = O_i, \forall i = 1, ..., k_{private}$. 
% This formulation has been proposed in benchmarks such as~\citet{chen2021evaluating, li2022competition, li2023taco, jain2024livecodebench, hendrycksapps2021, gulwani4foundations}. 
This setup is in contrast to math problems, where no additional information is given beyond the problem specification, and evaluation is done by exact matching on the final solution~\citep{li2024numinamath}.


% In this section, we formally introduce the problem setup and the ~\frameworkname~framework. %an experiment setup to configure the default setting that we will use in our final experiment.
% \joey{I wouldn't add the experiment setup in the methods section.}


%\noindent\textbf{Problem Setup} We consider coding problems that are clearly specified and unambiguous, as pointed out to be important in~\citet{chowdhury2024introducing}. In particular, we assume coding problems that include a small amount of input and output demonstrations, a common setup as~\citep{chen2021evaluating, li2022competition, li2023taco, jain2024livecodebench, hendrycksapps2021, gulwani4foundations}. We provide one such example in~\autoref{sec:appendix_example_code}. \joey{This paragraph doesn't actually say much. Instead, you might say something that is more detailed and provides greater contrast to the math setting.  In the programming setting we are given a detailed description of a function to implement along with a set of $k$? test input-output pairs and asked to produce a program that produces the same output for each test input.  The model then produces an implementation that is evaluated on a hidden set of unit-tests.  This is in contrast to the math setting where no additional information is given beyond the problem statement and evaluation is done by exact matching on the final solution.}

\subsection{The \frameworkname Framework}
The \frameworkname consists of two-stages: \emph{Generation}  and \emph{Selection}.
The generation stage combines repeated sampling to improve coverage%, the fraction of problems that could be solved, 
, with revision from public tests execution output to
improve the quality of %such diverse 
the samples. The selection stage features a test-assisted LLM-as-a-judge approach, which grounds LLM selection with code execution results.
%to provide further information 
%to enable more accurate LLM guided selection (~\autoref{sec:scale_selection}).

% \frameworkname~is a simple and effective three-stage approach. 
%\joey{I don't think you need the words simple and effective.  They are okay in the intro but here just say it is a three stage approach that combines sequential and parallel scaling with a verification process.  Then provide a high-level description of each of the three phases and how they work together.  It should be clear at the end that this is simple and in the eval you will prove it is effective.}
% It incorporates the advantage of parallel scaling by allowing the model to generate multiple solutions to improve coverage~\citep{brown2024large}, sequential scaling by allowing the model to revise a previous code solution by providing execution feedback on available public demonstration, and that of a verifier by choosing the best one. A high-level illustration can be found at~\autoref{fig:Design}. % In this section, we will introduce each stage, and our findings based on a development set to enable the default setting of~\frameworkname.

\subsubsection{Stage 1: Generation}
% \section{Scaling Parallel Sampling}
\label{sec:scale_parallel_samples}
In the generation stage, \frameworkname leverages the repeated sampling paradigm and leverages public tests execution result to ground revision. % For each sample, the LLM further revise its previous solution based on the execution result on public tests. Following ~\citet{chen2023teaching}, we implement this by executing
% using the SELF-DEBUGGING approach proposed by % \citet{chen2023teaching}. 
% \joey{Can you give a short description of how they defined self-debugging in the original paper. Then if there are any differences say how we implement self debugging here.  If they are identical then say "As in ..., we implement self-debugging by ..."}
Following similar implementation as in~\citet{chen2023teaching}, \frameworkname  generates $\mathbf{N}$ samples independently, and performs at most $\mathbf{R}$ rounds of revision with execution feedback from the set of public tests. For each sample, the revision procedure terminates if it passes all public tests or reaches the maximal debug round. We further experiments with additional revision from model generated tests, but do not found additional benefit in~\autoref{ssect:ablation_selfdebug}.
% We denote the $n^{th} (\in {1, ..., N})$ solution produced at the $r^{th} (\in {1, ... R})$ round as $S_{r}^{n}$. 
% For each sample, the SELF-DEBUGGING procedure terminates if the sample passes all public tests, or reaches the maximal debug round $\mathbf{R}$.


\subsubsection{Stage 2: Selection}
\label{sec:scale_selection}
In the selection stage, we need to select the best program from the $N$ candidate programs produced in the generation stage. However, since we have exhausted public tests in the Generation stage, we need to generate additional filtering step. We consider two prior paradigms, (1) LLM-as-a-judge based, which harnesses general pre-trained knowledge~\citep{zheng2023judging}, and (2) generated test based~\citep{li2022competition}, which leverages interpreter to ground selection. During exploration, we find that a naive LLM-as-a-judge approach that compares two code samples could hardly provide accurate selection because the LLM could hardly simulate the outcomes of such codes. On the other hand, a pure generated test based approach could hardly accurately select a sample because they can hardly predicts the test case accurately (\autoref{tab:diff_selection}).

%However, because all of the $N$ programs now pass the public tests, we need an additional filtering step to select the best program. 
% In addition, prior work has show that the public tests often have very little coverage of the problem. . % \joey{finish writing this to setup the problem solved in the selection stage and ideally emphasize why it is challenging (why can't you just ask an LLM to judge or just average or cluster the programs).}


Inspired these findings, we develop a hybrid selection method that uses LLM-as-a-judge framework, and together with test execution result to provide accurate grouding. Firstly, we prompt an LLM to generate a set of inputs, and group these $N$ samples into clusters, where samples in clusters have the same execution result on all generated inputs. Secondly, we select the best cluster by iteratively pairwise comparison between samples between clusters. For each sample comparison, we ask the LLM to generate a distinguishing input to separate these two samples, we execute the input to obtain the output, and ask the LLM to select the better one. We found that this selection strategy provides grounding to the LLM selection (see \autoref{sec:exp}), and is more reliable than majority voting-based methods.

\input{algorithm}

% we prompt a LLM to generate a set of inputs according to $\mathbf{P}$. Then, we execute these $\mathbf{N}$ samples and obtain their execution

% cluster the $\mathbf{N}$ candidates into clusters based

% Firstly, the $\mathbf{N}$ samples are clustered into a , based on a set of model generated inputs. 

% After Stage 2, there are N samples that needed to be selected. In this section, we consider several ways to do this selection, and propose our simple solution to better select candidates. We consider the following algorithms.

% \paragraph{Generated tests based} The most straightforward way to do selection is to do majority voting. Unlike math domains, where results are matched by exact match, in coding, we need to generate test inputs -> Generated test inputs + majority voting on the output. The other way is to do generated inputs and generated test outputs, also a popular choice~\citep{ehrlich2025codemonkeys}.

% \paragraph{LLM-as-a-judge based} This is often used in natural language as the way to select the better samples.


% Some ablation here - we find that generated tests + majority voting is not reliable because majority is wrong for hard problems. Using test outputs are also wrong because usually that assumes a strong model.

% On the other hand, LLM-as-a-judge can not found the correct one, because llm can hardly reason on code.

% Based on this, we develope a hybrid approach, shown in some figure, that first uses test inputs to cluster into several groups. then we use llm-as-a-judge. However, we do not simply use llm-as-a-judge, as we know it does not work. We let the llm to propose a test input that can potentially distinguish samples, execute it back, and then based on the results, do the selection, We found this consistently improve the result.\DL{Add figure, and a table here.}

